Optimized Preference-Aware Multi-path Video Streaming with Scalable Video Coding

Most client hosts are equipped with multiple network interfaces (e.g., WiFi and cellular networks). Simultaneous access of multiple interfaces can significantly improve the users' quality of experience (QoE) in video streaming. An intuitive approach to achieve it is to use Multi-path TCP (MPTCP). However, the deployment of MPTCP, especially with link preference, requires OS kernel update at both the client and server side, and a vast amount of commercial content providers do not support MPTCP. Thus, in this paper, we realize a multi-path video streaming algorithm in the application layer instead, by considering Scalable Video Coding (SVC), where each layer of every chunk can be fetched from only one of the orthogonal paths. We formulate the quality decisions of video chunks subject to the available bandwidth of the different paths, chunk deadlines, and link preferences as an optimization problem. The objective is to to optimize a QoE metric that maintains a tradeoff between maximizing the playback rate of every chunk and ensuring fairness among chunks. The QoE is a weighted some of the following metrics: skip/stall duration, average playback rate, and quality switching rate. However, the weights are chosen such that pushing more chunks to the same quality level is more preferable over any other choice. Even though the formulation is a non-convex discrete optimization, we show that the problem can be solved optimally with a polynomial complexity in some special cases. We further propose an online algorithm where several challenges including bandwidth prediction errors, are addressed. Extensive emulated experiments in a real testbed with real traces of public dataset reveal the robustness of our scheme and demonstrate its significant performance improvement compared to other multi-path algorithms.

==> conclusion.tex <==

\section{Conclusions}


This paper gives adaptive streaming algorithm for a  video encoded with Scalable Video Coding (SVC) over multiple paths, where each layer of every chunk can be fetched from only one of the paths. The problem for optimizing user's quality of experience (QoE) is formulated as a combinatorial optimization. It is shown that this combinatorial problem can be solved optimally with a complexity that is quadratic in the video length. Further, an online algorithm is proposed where 
several challenges including  bandwidth prediction
errors are addressed. Extensive simulations and emulations with real traces of public dataset reveal the robustness of our scheme and demonstrate its significant
performance improvement compared to other multi-path algorithms. 


==> emulation.tex <==
\section{Emulation Results}\label{sec:emu}

\begin{figure}
\centering
\vspace{-.2in}
\includegraphics[trim=0in 2in 0in 0in, clip,width=0.4\textwidth, height=2in]{emuSys.pdf}	
\vspace{-.3in}
 \caption{System Architecture for Emulation of MP-SVC.}
 \label{fig : emuSys}
% \vspace{.5in}
 \end{figure}


\begin{figure}
	\input{emuProfilesV2.tex}
	\vspace{-.2in}
 \caption{(a) Link 1 bandwidth profile, and (b) Link 2 bandwidth profile.}
\label{fig : emuProfiles}
\end{figure}


%\begin{figure}
%\centering
%\vspace{-.4in}
%\includegraphics[trim=0in 0in 0in 0in, clip,width=0.48\textwidth]{emuProfiles.eps}	
%\vspace{-.1in}
% \caption{(a) Link 1 bandwidth profile, and (b) Link 2 bandwidth profile.}
% \label{fig : emuProfiles}
% %\vspace{-.3in}
%\vspace{-.2in}
% \end{figure}
%

To complement our simulation results, we have built an emulation testbed, which is depicted in Fig.~\ref{fig : emuSys}. The server, and the client nodes are both running in a Linux machine with kernel version 2.6.32, 24 CPU cores, and 32MB memory. The server and client communicate with each other via the loopback interface using the default TCP variant, TCP CUBIC~\cite{ha2008cubic}. Two orthogonal links were created to emulate the behavior of the multi-path streaming. To fetch a layer of a chunk, the client sends a request for that layer to the server via one of the two links, determined by our algorithm, thus the server will send back the data packets of that chunk layer via the same link. The emulation ends when all chunks are received and played back. We record the received time, the playback time and the actual number of layers received for every chunk. To introduce bandwidth variations into the emulated experiments, we adopt \texttt{Dummynet}~\cite{dummynet} running on the client side, thus the incoming rates of the TCP packets from the server on the both links (i.e., 1 or 2) will be throttled according to the bandwidth datasets used. The bandwidths profile of the datasets for the both links are described in Section \ref{sec:eval}, from which one profile of each dataset is chosen and are depicted in Fig.~\ref{fig : emuProfiles}. 
The emulation results using these bandwidth profiles are compared with the simulation results, and the comparison is qualitatively similar for the other profiles. Thus, only the depicted profiles are used in this section.  The chosen bandwidth profiles have an overall max/mean/min values of 5.9, 1.68 and 0 Mbps for link $1$ (which has higher variance than link $2$), and 1, 0.88 and 0.65 Mbps for link $2$.
%\if 0
%\begin{figure}
%\centering
%\vspace{-.2in}
%\includegraphics[trim=0.4in 0in 0.25in 0in, clip,width=.48\textwidth]{em_vs_sim.eps}	
%\vspace{-.1in}
% \caption{Comparison of Emulation With Simulation results of MP-SVC, (a) Playback Quality CDF, and (b)  Playback Quality with time}
% \label{fig : emuVsSim}
% %\vspace{-.3in}
% \end{figure}
% \fi
 \begin{figure}
 \centering
\input{sim_vs_em_equal_skip}
\vspace{-.3in}
\caption{Simulation vs Emulation for equal priority skip based streaming (a) Quality CDF, and (b) Playback rate}
\label{fig : emuVsSim}
 \end{figure}
\begin{figure}
\centering
\input{sim_vs_em_pref_skip}
\vspace{-.3in}
\caption{Simulation vs Emulation for Link preference skip based streaming (a) Quality CDF, and (b) Playback rate}
\label{fig : emuVsSimPref}

 \end{figure}

 
For both simulation and emulation, we consider the parameters as described in Section \ref{sec:eval}. We note that the mean run time for the algorithm for a window size of 10 chunks (40 s) was 7.6 ms over a large number of runs for the different bandwidth profiles. This depicts the computational efficiency of the proposed algorithm. 

Figures \ref{fig : emuVsSim} and  \ref{fig : emuVsSimPref}  compare the playback quality of simulation and emulation for both equal priority and Link preference skip based streaming, respectively.  Figures \ref{fig : emuVsSim}-a and \ref{fig : emuVsSimPref}-a  plot the CDF of the playback quality, and Figures \ref{fig : emuVsSim}-b and  \ref{fig : emuVsSimPref}-b depict the playback bit rate in Mbps over time. From these figures, we note that the emulation results closely match the simulation results in terms of playback quality. Moreover,  the Link 1 usage achieved by emulation also matches the simulation results (not depicted in a figure). Therefore, the emulation results confirm the practicality of the proposed algorithm. 

%One more thing worth mentioning is that in the playback rate figures (Fig.~\ref{fig : emuVsSim}-b and Fig.~\ref{fig : emuVsSimPref}-b), we see that the playback rate curve starts at zero since the startup delay is 5s, so first chunk is played after 5 seconds. Moreover, as it was explained in section.~ \ref{sec:bw_err}, the first two chunks are fetched at base layer quality, and that is why we see the playback rate starts at 0.6Mbps (BL rate).

%The chosen bandwidth profiles have the first link bandwidth higher in the start, and decreases later on. This impacts the quality decisions, where the earlier chunks are fetched at higher quality which degrades later. Both the simulation and emulation results show similar drops and increases of rates. 

% are high at the beginning and runs low close to the end, the quality decisions up to the chunk numbered 200 were fetched at highest quality level for both simulation and emulation, and when the average bandwidth dropped we started to see the algorithm changing the requesting policy, and running into quality switches and skips in the same manner for both emulation and simulation.


==> noskipsims.tex <==
\subsection{No-Skip Based MP-SVC Algorithm}
\label{sec:eval_noskip}
\if 0
\begin{figure*}
%\vspace{-.1in}
\centering
\begin{minipage}{.49\textwidth}
\includegraphics[trim=1.2in 0in .5in 0.5in, clip,  width=\textwidth, height=3in]{./multiPath_results/noSkip_results.eps}	
\caption{No-Skip based streaming results on Dataset1: (a) layer distribution, (b) CDF of average playback rate, and (c) CDF of re-buffering time.}
% \label{fig : noSkipComp}
%\vspace{-.3in}
%\end{figure}
\end{minipage}
\begin{minipage}{.49\textwidth}
\centering
%\begin{figure}
%\vspace{-.1in}
\includegraphics[trim=1.2in 0in .5in 0.5in, clip,  width=\textwidth, height=3in]{./multiPath_results/noSkip_results_fcc.eps}	

\caption{No-Skip based streaming results on Dataset2: (a) layer distribution, (b) CDF of average playback rate, and (c) CDF of re-buffering time.}
 \label{fig : noSkipComp2}
%\vspace{-.3in}
\end{minipage}
\end{figure*}
\fi

\begin{figure}
\vspace{-.15in}
\centering
\includegraphics[trim=1in 0in .5in 0.5in, clip,  width=.5\textwidth]{./multiPath_results/noSkip_results.eps}	
\vspace{-.7in}
\caption{No-Skip based streaming results: (a) layer distribution, (b) CDF of average playback rate, and (c) CDF of re-buffering time.}
 \label{fig : noSkipComp}
%\vspace{-.3in}
%\end{figure}
\vspace{-.2in}
\end{figure}

%{\bf mention buffer threshold}
%Since the algorithms are similar, the results are qualitatively similar to those described in Section \ref{sec:eval_skip}

In this subsection, we evaluate our proposed algorithm for the No-Skip based scenario. The initial startup delay is chosen to be the minimum of 1s and the download time of the first chunk while the other parameters are the same as in the skip-based version. The results are shown in Fig.~\ref{fig : noSkipComp}. The main difference in the no-skip version is that since there are no skips, the video may have multiple stalls. Thus, in Fig.~\ref{fig : noSkipComp}, we evaluate the duration of stalls (re-buffering time) as an additional metric. We omit the layer switching rate since the results are qualitatively similar to skip version ones. 

We first note that MPTCP-SVC in general performs better than MP-SVC in term of avoiding stalls since multipath TCP can be used which gives better flexibility as compared to obtaining a layer only on one path.  We see in Fig.~\ref{fig : noSkipComp} that the stall duration for MP-SVC is slightly higher as compared to MPTCP-SVC. The probability mass function of the qualities at which different chunks are obtained, and the  CDF of the average video playback rate results show  that the performance of MP-SVC  is close to that of  MPTCP-SVC. 

Further, MP-SVC and MPTCP-SVC significantly outperform both MP-BBA, and MPTCP-BBA in term the average playback rate. They are about $38\%$, and $29\%$ higher than MP-BBA and MPTCP-BBA, respectively. Even though MSPlayer achieves the highest average playback rate, it runs into stall of duration of  more than a minute  for $50\%$ of the traces. MP-SVC and MPTCP-SVC  achieve low number of stalls, no stalls for about $80\%$ of the traces (similar to offline results), and less than $30s$ and $7$s for $90\%$ of the traces, respectively. %Moreover, the stall duration of MP-SVC and MPTCP-SVC can be reduced further if $B_{min}$ is increased (for the current simulation, $B_{min}=0$). 
 Thus, MP-SVC and MPTCP-SVC achieve a better tradeoff between the average playback rate and stall durations. 

%We see how MP-SVC, and MPTCP-SVC trade-off high average rate with low number of stalls. Without setting lower buffer threshold, they achieve low number of stalls,  less than $20s$ and $7$s for $99\%$ of the traces respectively. This stall duration could have been reduced with a cost of lower playback rate if we set a lower buffer threshold, so if the buffer runs bellow that threshold, chunks are fetched at base layer. %Finally, MP-BBA and MPTCP-BBA run into the lowest number of stalls but the cost is achieving significantly lower average playback rate with compare to MP-SVC and MPTCP-SVC.

%The only difference of the structure of the figures with compare to skip version is that we have replaced the layer switching rate subplot with stall (re-buffering time) CDF plot Fig.~\ref{fig : noSkipComp}-c and Fig.~\ref{fig : noSkipComp2}-c. We omit the layer switching rate because the results are very similar to skip version case.. The key observations from Fig.~\ref{fig : noSkipComp} and Fig.~\ref{fig : noSkipComp2} are:

%

%\begin{itemize}
%\item MP-SVC neither require any kernel modification nor network worries of blocking the packets, and yet achieve similar results as MPTCP-SVC. We clearly see that the results of offline MP-SVC is very close to offline MPTCP-SVC which requires MPTCP installed at both client and server. The difference is negligible. Moreover, the online MP-SVC is also very close to online MPTCP-SVC, and both are the closest to the offline MPTCP-SVC which is the best that can be achievable. 
%\item No-Skip results confirms the skip based results in stating that the MPTCP win over application layer is very negligible. We clearly see from both figures Fig.~\ref{fig : noSkipComp} and Fig.~\ref{fig : noSkipComp2} that MP-SVC and MPTCP-SVC have very similar results.

%\item MPTCP-SVC incur very negligible stall duration with compare to the offline algorithm, and MP-SVC incur little bit higher stalls in the high average regime (HSDPA dataset). However, MP-SVC could reduce this stall duration by setting a lower buffer threshold, so if the buffer occupancy is lower than that threshold, the decision is modified such that all chunks are fetched at base layer quality. In fact we did that, and we reduced the stall duration very significantly with some loss in average playback quality. {\bf: I can have results where we have lower buffer threshold, so we have one more curve}
%\item Both MP-SVC and MPTCP-SVC, achieve high average playback rate. The average playback rate is, about $33\%$, and $28\%$ higher with compare to MP-BBA, and MPTCP-BBA, respectively on HSDPA dataset, and  $30\%$, $22\%$, and $21\%$ higher with compare to MP-BBA, MPTCP-BBA, and MSPlayer on FCC dataset respectively.

%\item  Both MP-SVC and MPTCP-SVC achieve the high average and low number of skips with very competitive layer switching rate. As Fig.~\ref{fig : BComp}-c and Fig.~\ref{fig : BComp2}-c show, the CDF curve of the switching rate of MPSVC is similar to MP-BBA on HSDPA and they beat it in the FCC data because the average bandwidth of FCC dataset is low, so MP-BBA will struggle in switching between before and after the lower threshold (the startup and the linear decision regions). MP-SVC achieves very low layer switching rate and very close to the offline algorithm on FCC data with being $99\%$ of the time less than $4\%$. It is slightly higher on HSDPA dataset with being less than $20\%$ for $99\%$ of the time.

%\item MSPlayer achieve high average playback rate on high average regime (HSDPA dataset), but the cost is very expensive. It runs into so many stall durations. Fig.~\ref{fig : noSkipComp}-c shows that MSPlayer runs into about 1 minute of stall in more than $50\%$ of the traces. Moreover, it struggles with both low average playback rate and high stall duration at low average regime (FCC dataset). This clearly shows that to achieve a good trade -off between minimizing stalls and maximizing average quality both current buffer and prediction of future bandwidth are required and this what MP-SVC algorithm is doing.

%\item MP-BBA and MPTCP-BBA acheive very low re-buffering time, but the cost is significantly lower average playback rate with compare to what can theoretically be achieved.

%of over all traces. both achieve $18\%$ and $$ improvement with compare to BBA, $$ and $$ with compare to MPTCP-BBA, and $$ and $$ with compare to MSPlayer in HSDPA and FCC datasets respectively. 
%\end{itemize} 



==> optimal.tex <==
\subsection{Optimality of the MP-SVC}\label{optim_skip}

In this section, we prove that the proposed algorithm achieves the optimal solution of problem (\ref{equ:eq1}-\ref{equ:c7eq1}). The detailed proofs are provided in Section \ref{proof_skip}. The following result shows that the proposed algorithm minimizes the number of skips for a given layer among all the other algorithms which fetches the same quality levels up to the immediate next lower layer. %maximizes the number of chunks at least in the base layer obtained in any layer given the decisions of the previous layers. 

\begin{lemma}%{Theorem}
Given size decisions up to ($n-1$)th layer ($Z_{0,....,n-1}$), remaining bandwidth, and $deadline(i)$ for every chunk $i$, the proposed algorithm achieves the minimum number of $n$th layer skips (or obtains the maximum number of chunks at layer $n$) as compared to any feasible algorithm which fetches the same layers of every chunk up to layer $n-1$.
 \label{lem:skip1} 
\end{lemma}

Intuitively, the proposed algorithm pushes all the skips as early as possible since the earlier chunks will be closer to their deadlines, so skipping those will offer more bandwidth to the later ones, minimize the number of current layer skips, and maximize the number of candidate chunks to the next layer.
The next result demonstrates that the proposed algorithm leaves the maximum possible bandwidth before the deadline of every chunk that is a candidate (has all previous layers fetched) to the next layer.% in order to fetch its the next layer. 

\begin{lemma}%{Theorem}
Among all algorithms with the same number of $n$th layer skips, the proposed algorithm leaves the largest possible bandwidth for fetching the ($n+1$)th layer of every candidate chunk before its deadline. In other words, the proposed algorithm maximizes the resources to the higher layer among all algorithms that have same decisions up to the current layer.

%\textcolor{red}{I think this lemma needs to be re-written in a better way. We leave more bandwidth for every chunk before its deadline, so we maximize the number of candidates to the next layer.} %fetch the same number of current layer chunks . \textcolor{red}{since same number of current layer does not mean same policy up to the current layer, I think the last statement should be replaced with this one: In other words, the proposed algorithm maximizes the resources to the higher layer among all algorithms that have same decisions up to the current layer} 
%maximizes the number of candidate chunks to the next layer.%has optimal $n$th layer skip pattern
\label{lem:skip2}
\end{lemma}

Intuitively, our proposed algorithm optimizes the bandwidth resources to make more resources available for later layers. This is essential for optimality of the algorithm since the decisions for the higher layers depend on the decisions of the lower layers. Thus, if the decision of the lower layer does not help giving more resources for the higher layers, the algorithm will not be optimal.   Using Lemma \ref{lem:skip1} and Lemma \ref{lem:skip2}, the following result shows the optimality of MP-SVC algorithm in solving problem~(\ref{equ:eq1}-\ref{equ:c7eq1}).

\begin{theorem}	
Up to a given enhancement layer
 $M, M \geq 0$, if $Z_{m,i}^*$ is the  size of every layer $m \leq M$ of chunk $i$ that is found by running MP-SVC algorithm, and $Z_{m,i}^\prime$ is a size that is found by any other feasible algorithm such that all constraints are satisfied, then the following holds when $\gamma$ satisfies \eqref{basic_gamma_1}.%for any $0<\gamma \ll 1$. %and $\sum_{j > k}\gamma^j \sum_i Z_{j,i} \ll \gamma^k  Z_{k,1}$.
\begin{equation}
 \sum_{m=0}^M \gamma^m\sum_{i=1}^{C} Z_{m,i}^\prime \leq \sum_{m=0}^{M} \gamma^m\sum_{i=1}^{C} Z_{m,i}^*.
\label{thm:thm}
\end{equation}
In other words, MP-SVC finds the optimal solution to the optimization problem~(\ref{equ:eq1}-\ref{equ:c7eq1}) when $\gamma$ satisfies \eqref{basic_gamma_1}.% \textcolor{red}{and M=N}. %$0<\gamma \ll 1$.% and $\sum_{j > k}\gamma^j \sum_i Z_{j,i} \ll \gamma^k Z_{k,1}$.
\label{theorem: theorem11}
\end{theorem}
Intuitively, note that MP-SVC first fetches the lower quality level of all the chunks before fetching the next higher levels. Thus, the QoE attained is higher. It also prefers the excess bandwidth to be utilized for fetching higher quality layers of the later chunks. Finally, since MP-SVC minimizes the skips, thus, it is the optimal. 



%\textbf{Can you give any intuition why this is optimal?}


==> pref_formulation.tex <==
\section{Offline Problem Formulation For SVC Video Streaming with Link Preference}\label{apdx_pref}

In addition to the objectives mentioned without link preference, we further consider minimization of the link $1$ usage. In order to account for the third objective of minimization of link $1$, we consider a parameter $m\in \{0, \cdots, N\}$ indicating that the link $1$ should not be used to obtain chunks above layer $m$. This will help using link $1$ to help improve getting lower layers while not over-using it to achieve higher layers. Further, among different schemes that obtains same number of chunks till layer $m$, we wish to minimize the usage of link $1$. For $m=0$, this implies that link $1$ is only used to avoid skips and not to fetch any enhancement layers. Further, link $1$ is used only if necessary to reduce skips, when link $2$ is not sufficient to obtain the optimal number of base layer chunks. In order to account for these properties of the usage of link $1$, we subtract $D \gamma^{m+1}  \sum_{n=0}^{N}\sum_{i=1}^{C}\sum_{j=1}^{(C-1)L+s} z_n^{(1)}(i,j)$ from the objective for $\gamma$, where $D\ge 2$ satisfies

\begin{equation}
C\sum_{j=1}^{N-a} \gamma^j r_{a+j} + D \gamma^{m+1-a}r_a < r_a, \  \text{  for } a= 0, \cdots, m,  \label{basic_gamma_2}
\end{equation}
and
\begin{equation}
D  \Delta_m  > C \sum_{n=m+1}^N \gamma^{n-m-1} r_n,  \label{basic_gamma_3}
\end{equation}
where 
\begin{equation}
\Delta_m  \triangleq \min\{x: x>0, x= \sum_{i=0}^m c_i r_i, c_i \in \{-C, \cdots, C\} \}
\end{equation}


\eqref{basic_gamma_2}  is stronger than \eqref{basic_gamma_1} for $a\le m$ and for $a=m$ also gives $D<1/\gamma$. The constraint \eqref{basic_gamma_2} says that the cost of link $1$ does not constrain fetching of the lower layers, while the constraint \eqref{basic_gamma_3} wishes to limit the use of link $1$ if it does not increase the qualities of layers up to $m$. With these conditions on $D$ and $\gamma$, we will show that the above mentioned properties for the usage of link $1$ are satisfied. Overall, the multi-path SVC layer scheduling problem with the knowledge of future bandwidth information can be formulated as follows.

\begin{eqnarray}
maximize \sum_{n=0}^{N}\sum_{i=1}^{C} \Bigg(\gamma^nZ_{n,i}- D \gamma^{m+1} \sum_{j=1}^{(C-1)L+s} z_n^{(1)}(i,j)\Bigg) %- \lambda \sum_{j=1}^{deadline(C)} B(j)^{(2)}  \Bigg)
%\sum_{n=0}^{N} \lambda_n \gamma^n \sum_{i=1}^{C}\beta^i B_{n,i}^{(2)}  \Bigg)
\label{equ:eqap1}
\end{eqnarray}
%\vspace{-.1in}

subject to \eqref{equ:c2eq1}-\eqref{equ:c7eq1}
\begin{eqnarray}
\text{Variables:}&& z_n^{(2)}(i,j), z_n^{(1)}(i,j),  Z_{n,i} \ \ \  \forall   i = 1, \cdots, C, \nonumber \\&& j = 1, \cdots, (C-1)L+s, n = 0, \cdots, N \nonumber
\end{eqnarray}



We will now show that the problem formulation does not fetch any chunk using Link 1 at a layer greater than $m$. 
\begin{lemma}\label{lem_nohigher}
	None of the layers is fetched using link $1$ for any layer greater than $m$. More precisely,  $\sum_{j=1}^{(i-1)L+s} z_n^{(1)}(i,j)=0$ for all $i\in \{1, \cdots, C\}$ and $n>m$. 
\end{lemma}
\begin{proof}
	Suppose that layer $n>m$ of chunk $i$ is fetched using link $1$. The additional utility obtained by fetching layer $n$ and higher is at most $\sum_{k=n}^{N} \gamma^k r_k$ which is lower than the loss of using Link 1 for layer $n$, which is greater than $2 \gamma^{m+1}r_n$ using \eqref{basic_gamma_1}. Thus, it is better not to fetch chunk $i$ at layers $n$ and higher if this layer is to be fetched using link $1$.
\end{proof}



Thus,  Link $1$ can only be used to fetch chunks at the layers till layer $m$. However, among any two strategies that achieve the same number of chunks at all layers till layer $m$, the proposed problem formulation will choose the one with lower Link 1 usage. This is given in the following lemma. 


\begin{lemma}\label{lem_lower}
	Among two strategies with the same layers fetched for every chunk for layers from $0$ to $m$, the one that obtains lower content over link $1$ is preferred.
\end{lemma}
\begin{proof}
	For the same possible chunks till layer $m$, the minimum extra usage of link $1$ is $\Delta$. Thus, as long as the additional cost of this Link 1 usage is more than all the benefits of the layers above $m$, the cost will outweigh the benefit. Since this holds by \eqref{basic_gamma_3}, the result holds.
\end{proof}

Finally, we note that choosing link 1 for layers from $0$ to $m$ will have positive utility since $D<1/\gamma$. Finally, we need to show that if an extra chunk can be obtained at a layer $n\le m$, the above problem will not be constrained by the cost of using link $1$. This is satisfied due to \eqref{basic_gamma_2}. More formally, the following holds. 

\begin{lemma}\label{lem_lower_unc}
	Among two strategies with the same number of chunks at layer $0, \cdots, k$ for $k<m$, the strategy that obtains the largest number of chunks in layer $k+1$ achieves better objective.
\end{lemma}
%\textcolor{red}{Why this is a lemma?, and if you think it should be a lemma, where is the proof?}
Thus, we see that the utility function for the above choice of range of $(D, \gamma)$ satisfies the properties needed for the formulation. 

Even though we do not have a general algorithm that optimizes this proposed formulation for any value of $m$, the proposed algorithm MP-Pref-SVC in Section \ref{sec:pref} is optimal when $m=0$. Thus, when the objective is only to use link $1$ to avoid skips, the proposed algorithm is optimal. This is easy to see using Lemma \ref{lem_lower} that the proposed algorithm satisfies this condition. Thus, all the conditions of optimality of the additional cost function are satisfied. The key reason this does not hold for general $m$ is the greedy policy of Link1-Save algorithm in Algorithm \ref{Link1-Save }. It is not necessary for a general $m$ that this strategy will use minimum amount of link $1$. 

Finally, we note that when MPTCP can be used, the key difference is that the constraint \ref{equ:c5eq1} is removed. Thus, when partial fetching is allowed, the modification of Link1-Save  will use minimum link $1$ and thus all the conditions are satisfied for any $m$. This proves that the proposed algorithm is optimal for all values of $m$, when MPTCP can be used. We further note that the decisions made using this algorithm can be used for both SVC and AVC when MPTCP can be used.

==> skip_optimality.tex <==
\section{Optimality of No Skip Based  Streaming Algorithm}\label{no_skip_apdx}
%\textcolor{red}{I think the this section except the proof should be moved to the main text} 
The following lemma states formally that the No-Skip MP-SVC algorithm achieves the minimum stall duration such that all chunks are at least fetched at base layer quality.

\begin{lemma}
If $deadline^*(C)$ is the deadline of the last chunk ($C$) that was found using No-skip MP-SVC algorithm such that all chunks can be at least delivered at base layer quality, and $deadline^\prime(C)$ is the deadline of the chunk ($C$) that was found using any other algorithm, then:\\
$$deadline^\prime(C) \geq deadline^*(C).$$
In other words, No-Skip MP-SVC achieves the minimum stall duration such that all chunks are fetched at least at base layer quality.
%The deadline of chunk $i$ that is found by no skip base layer forward algorithm is the maximum deadline such that stall duration up to chunk $i$ playback time is at its minimum.
\end{lemma}
\begin{proof}
The proposed algorithm is a greedy algorithm that only adds to the deadline if there must be a skip due to not enough bandwidth. Further, the algorithm fetches all the chunks at only base layer quality which would have the lowest possible fetching times. Due to this greedy nature, no other algorithm can fetch all the chunks before those obtained by this greedy algorithm. 
\end{proof}

Having shown the minimum stall durations, Theorem \ref{theorem: theorem11} shows that the MP-SVC algorithm is optimal for the  proposed No-Skip problem when $\gamma$ satisfies \eqref{basic_gamma_1}. 



==> skipperfect-copy-copy.tex <==
\section{MP-SVC Algorithm}\label{skipalgo}
 In this section, we describe the proposed algorithm for skip-based streaming. To develop the algorithm, we first consider the offline algorithm in which the bandwidth is perfectly known for the whole period of the video. We first describe the algorithm when both links can be used without preference, and we refer to this algorithm as ``Offline Multi-Path SVC Algorithm" (Offline MP-SVC). This algorithm is, then, extended to the Preference-Aware case in which link 1 is more preferable and link 2 can only be used to fetch up to a certain layer. We refer to this algorithm as ?Offline Pref-MP-SVC?. We will show that Offline Pref-MP-SVC achieves the optimal solution of the proposed algorithm when link s can be used only to avoid skips ($n_2=0$). Finally, we propose an online algorithm (Online Pref/No-Pref MP-SVC) in which more practical assumptions are considered, such as short bandwidth prediction with prediction error and finite buffer size.
%In this section, we consider the case where $m=N$. We will first ignore $D$, by having $D=0$ and then explain the modification step accounting for the cost of the link $1$. Intuitively, based on Lemma\ref{lem_lower_unc}, obtaining the chunk qualities does not depend on $D$. Thus, we will first determine the qualities of the different chunks. Then, based on Lemma 
% \textcolor{red}{In the description of the algorithm, we do not explain the intuition behind starting from back. I think, we need to intuitively explain that.}
\subsection{MP-SVC Algorithm}\label{skipalgoEqual}
 In this section, we describe our 
 No-Preference based algorithm (Offline MP-SVC), which is summarized in
Algorithm \ref{algo:mpsvc}. The algorithm initially calculates the cumulative bandwidth of every second $j$ and link $r^{(k)}(j)$ (Line xx). Then, it makes the decision for the base layer, \ie which chunks to be skipped and which to be fetched. Moreover, the algorithm decides which link will be used to fetch the base layer of every chunk that has been decided to be fetched. The algorithm performs forward scan and finds the maximum number of chunks that can be fetched before the deadline of every chunk $i$ ($V(i)$). The maximum number of chunks that can be fetched before the deadline of the $i^{th}$ chunk is: $V(i)=\sum_{k=1}^2 \floor{r^k(deadline(i)}$(line 5). Therefore, if at the deadline of the $i^{th}$ chunk $V(i) < i$, there must be skips, the total number of skips will be incremented by $i-V(i)$(line xx). If there are $A$ skips, the algorithm will always skip the first $A$ chunks since they are the closest to their deadlines. Thus, skipping them will offer a bandwidth that can be used by all remaining chunks to increase their quality to the next layer. This choice maximizes the total available bandwidth for the later chunks. %Note that the number of skips could increase if the maximum contribution of all users is used before downloading all chunks.

Conseqently, the algorithm performs backward scan per chunk starting from the first chunk that was decided to be fetched by calling Algorithm 2 (line 21). The backward scan simulates fetching every chunk $i$ starting from its deadline and by every link that has $r^{(k)}(deadline(i)) \geq Y_0$(Lines 16, 17, and 20). The algorithm computes the residual total bandwidth that will remain. The link choice that maximizes the residual total bandwidth is chosen to fetch chunk $i$ as shown in Algorithm 2. Note that the link over which the chunk $i$ will be fetched is the one that gives the maximum amount of total available bandwidth over all links before the deadline of chunk numbered $i-1$.  For example, consider that there are only two links. Also, consider that fetching the $i^{th}$ chunk by user 1 results in using  $x$ amount of the bandwidth before the deadline of $i-1^{th}$ chunk while fetching the $i^{th}$ chunk by user 2 results in using  $y$ amount of the bandwidth before the deadline of $i-1^{th}$ chunk. Then, the first link will be chosen to fetch the chunk $i$ if $x<y$. The objective is to free as much as possible of early bandwidth since it will help more chunks to fetch their higher layers because it comes before their deadlines. 

%Once the base layer decision is taken, the algorithm sequentially decides to fetch the enhancement layers. %in a similar fashion.

{\bf Enhancement layer modifications}: The algorithm proceeds in performing forward-backward scan per enhancement layer in order. The bandwidth is now modified to be the remaining bandwidth after excluding whatever has been reserved to fetch lower layers (Line 7 in Algorithm 2).  Also note that $n^{th}$ layer for a chunk is not fetched if its $n-1^{th}$ layer was not fetched (Line 18 in Algorithm \ref{algo:mpsvc}).

\begin{figure}
		%\vspace{-.15in}
    \scalebox{0.95}{
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
			\small
				\begin{algorithmic}[1]
					%\vspace{-.05in}
				\STATE {\bf Input:}  $\mathbf{Y}=\{Y_n\forall n\}$, $L$, $s$, $C$, $U$, $\mathbf{B}_{u}=\{B_{u}(j)\forall j\}$, $u=1,..,U$. 
				\STATE {\bf Output:} $I^{(u)}_{n}$, $n=0,...,N$: set containing the indices of the chunks that can have their $n$th layer fetched by user $u$.	
								
    \STATE  $deadline(i)=(i-1)L+s, \quad \forall i$ 
	\STATE  $r^{(u)}(j)=\sum_{j^\prime=1}^{j} B_{u}(j^\prime)$, $j=1,....deadline(C)$, $u=1,..,U$
	\STATE $V_i=\sum_{u=1}^U\floor{r^{(u)}(deadline(i)}$: The total number of chunks that can be fetched before the deadline of the $i$-th chunk.
	
    \FOR{each layer $n = 0, \cdots, N$}   
    \STATE $skip=0$
     \FOR{$i=1:C$}
       \IF{$V(i) < i$}
       	\STATE $skip=skip+(i-V(i))$
	\ENDIF
      \ENDFOR
        \STATE Skip the first $skip$ chunks.
        \STATE $i^\prime=$the index of the first chunk to fetch
      % \STATE $j_{1}=j_{2}=....=j_{U}=deadline(C)$
     
    %\FOR{$u=1:U$}
     %{\bf j not defined - need efficient loop - should be also outside $n$ loop. }
    % available bandwidth on lte connection up to time $j, \forall j$
    \FOR{$i=i^\prime:C$}
    \STATE $j_u =deadline(i),\forall u=1....U$
   \STATE $r^u(j_u) =\min(r^u(j_u), \eta_u),\forall u=1....U$
    	\IF{($n=0$ or $i \in \{I_{n-1}^{(1)} \cup I_{n-1}^{(2)}\cup....\cup I_{n-1}^{(U)}\})$}
    		\IF{$max(r^{(1)}(j_1),...., r^{(U)}(j_U)) \geq Y_n$}
		\IF{$r^u(j_u) > Y_n$}
      			\STATE $[R^{(u)},B2_{u}]= Backward(u,i, j_u, \{r^{(u)}(j)\forall j\}, \mathbf{B}_{u}, Y_n,\eta_u^k)$,$\forall u$
      			\STATE $tmp(u)=R^{(u)}(deadline(i-1))+\sum_{u^\prime=1, u^\prime \neq u}^{U} r^{(u^\prime)}(deadline(i-1))$, $u=1, 2,...U$
			\ELSE
			\STATE $tmp(u)=0$
			\ENDIF
			\STATE $u_{max} = max \big( tmp^{(u)}\big)$
			\STATE $U_{max} \leftarrow$ users with $u_{max}$
      			\STATE $u_1 \leftarrow$ pick a user from $U_{max}$ randomly with uniform distribution
      			\IF { $(r^{(u_1)}(deadline(i)) \geq Y_n)$}
      				\STATE $I_n^{(u_1)}=I_n^{(u_1)} \cup i$, $\mathbf{B}_{(u_1)}=B2_{(u_1)}$
      				\STATE $r^{(u_1)} =R^{(u_1)}$, $Y_n=0$
				%\STATE $Y_n=0$				
      			\ENDIF
			%\ELSE
			%\STATE $Y=move()$
      		\ENDIF
	\ENDIF
      \ENDFOR
     \ENDFOR
   				\end{algorithmic}
				\caption{Offline No-Pref GroupCast Algorithm }\label{algo:mpsvc}
			\end{algorithm}
		\end{minipage}
	}
		%\vspace{-.55in}
	\end{figure}




\begin{figure}
		%\vspace{-.6in}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:} $u,i, j, r, B, Y_n$
					\STATE {\bf Output:} $R$ is the residual cumulative bandwidth at different times after fetching chunk $i$, $B2$ is the residual bandwidth after accounting for fetching of chunk $i$ 
    \STATE {\bf Initialization:}
    \STATE $i=C$
     \WHILE {($Y_n > 0$)}

            \STATE $fetched=min(B(j), Y_n)$ 
            \STATE $B(j)=B(j)-fetched$, $r(j)=r(j)-fetched$
            \STATE $Y_n(i)=Y_n(i)-fetched$
	   \STATE {\bf if } {$(B(j)=0)$} {\bf then }  $j=j-1$            	
    \STATE $R=r$, $B2=B$        
\ENDWHILE
				\end{algorithmic}
				\caption { Backward Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}
	
	
\if0	
\begin{figure*}
%\vspace{-.15in}
\centering
\includegraphics[trim=0.3in 0in .1in 0in, clip,  width=.48\textwidth]{./bwTrace.pdf}
\includegraphics[trim=0.3in 0.1in .1in 0in, clip,  width=.48\textwidth]{./bl.pdf}	
\includegraphics[trim=0.3in 3in 3in 0in, clip,  width=.48\textwidth]{./e1.pdf}	
\includegraphics[trim=0.3in 0.1in .1in 0in, clip,  width=.48\textwidth]{./fetching.pdf}	
%\vspace{-.7in}
 \vspace{-.3in}
 %\caption{ Skip based Streaming without link preference: (a) layer distribution, and (b) CDF of layer switching rate.}
 %\label{fig : BCompeq}
% \vspace{-.1in}
\end{figure*}
\fi


	
{\bf Example: } In this example, we assume the bandwidth trace of both links are as shown in~Fig~\ref{fig:example}. Moreover, as shown in the figure, the video is an SVC encoded video consists of 10 chunks. The video is encoded into 1 Base Layer($BL$) and 1 Enhancement Layer($E_1$). The $BL$ and $E_1$ sizes are $2Mb$, and $1Mb$ respectively. \ie  $Y_0=2Mb$, and the $Y_1=1Mb$.



 

 \begin{theorem}%{Theorem}
Given size decisions up to $n-1^{th}$ layer ($Z_{0,i}, \cdots,Z_{n-1,i}$, for all $i$), remaining bandwidth, and $deadline(i)$ for every chunk $i$, the proposed algorithm achieves the minimum number of $n^{th}$ layer skips (or obtains the maximum number of chunks at layer $n$) as compared to any feasible algorithm which fetches the same layers of every chunk up to layer $n-1$.
 \label{lem:skip1} 
\end{theorem}
\begin{proof}
Proof is provided in Appendix \ref{proofskipl1}.
\end{proof}












\if0

This algorithm first makes the decisions for the base layer (i.e., which chunks to be skipped, and which to be fetched over link $k$, $k \in\{1,2\}$). The algorithm performs backward scan starting from the deadline of the last chunk (line 7) and checks the possibility of fetching chunks according to the available bandwidth (line 10, where $r^{(k)}(j)$ is the cumulative available bandwidth of the  link $k$ up to the $j$th time slot). Given the decisions of chunks $i+1, \cdots, L$, we wish to decide which of the two links should chunk $i$ be fetched at, such that the objective function is maximized while satisfying the constraints. For both choices of links at which chunk $i$ can be fetched, we compute the residual total bandwidth (sum of the bandwidths of the two links) that will remain for the download of chunks $1, \cdots, i-1$. The link choice that maximizes the residual total bandwidth is chosen to fetch chunk $i$ (Algorithm 2). 

 
 
 %\textcolor{red}{for the case when $\lambda=0$, so both links can be used without preferring  one over the other, and then we will for any value of $\lambda$.} 
 
 %which is summarized in Algorithm \ref{algo:mpsvc}. 
%our algorithm works from the lowest (i.e the base) to the highest enhancement layer, and processes each layer separately. It performs backward scans (explained below) at each layer given the decisions of the previous layers.
%\subsubsection{Efficient Quadratic-time Solution}\label{skipalgo}

%\textcolor{red}{In equal priority}, MP-SVC algorithm (Algorithm \ref{algo:mpsvc}) 


Note that the algorithm is similar to  dynamic programming, where the algorithm decides the quality at which the chunks will be fetched starting from the last one. The link over which the chunk $i$ is fetched is the one that gives the maximum amount of total available bandwidth over the two links before the deadline of chunk numbered $i-1$.  For example, consider that  fetching the $i$-th chunk over the  link 1 results in using  $x$ amount of the bandwidth before the deadline of $i-1$-th chunk while fetching the $i$th chunk over  link 2 results in using  $y$ amount of the bandwidth before the deadline of $i-1$th chunk. Then, the first link will be chosen to fetch the chunk $i$ if $x<y$. 

%The backward algorithm (Algorithm 2) starts from fetching the base layer of each chunk $i$. It will then decide the link which leaves more bandwidth for remaining chunks (less than $i$) to fetch the layer using the link. Once the base layer decision is taken, the algorithm sequentially decides to fetch the enhancement layers using one of the links in a similar fashion. %in each of the links, and the one that leaves more bandwidth for the remaining chunks (chunks < $i$) will be assigned this layer to fetch.  The algorithm takes as input, the starting time slot of fetching layer $n$ of chunk $i$ on  the link $wifi/lte$ ($j_1/j_2$), the predicted bandwidth $B^{(1)}/B^{(2)}$, the cumulative predicted bandwidth $r^{(1)}/r^{(2)}$, and the chunk size $Y_n$, ad checks the possibility of fetching it over that link. If the remaining bandwidth of any of the links is less than a chunk size, then that link is excluded (lines 9-21, and 24-26). Otherwise, the algorithm compares the total bandwidth available for the remaining chunks (chunks $< i$) if the current chunk is fetched over WiFi with its value if the chunk is fetched over LTE link using the returns of the backward algorithm ($j_3/j_4$: the time slot in which chunk $i$ is fully downloaded over link $wifi/lte$, $B1/B2$: the remaining bandwidth of the link wifi/let, $r_1/r_2$: the remaining cumulative bandwidth up to $j_3/j_4$ of the link $wifi/lte$, lines 29-37), and the link that leaves more bandwidth before the deadline of $i-1$ will be assigned this layer to fetch.} %\textbf{Difficult to parse. Can you elaborate more?} \textbf{Arnob: I tried to simplify it further, but I am not sure if it is now better, plz read and let me know what you think}


Once the base layer decision is taken, the algorithm sequentially decides to fetch the enhancement layers. %in a similar fashion.

{\bf Enhancement layer modifications}: The algorithm proceeds in a similar fashion to decide for the next higher layer and so on.  The bandwidth is now modified to be the remaining bandwidth after excluding whatever used to fetch lower layers (line 10, Algorithm 2).  Also note that $n$th layer for a chunk is not fetched if its $(n-1)$th layer was not fetched (line 9, Algorithm \ref{algo:mpsvc}).

\begin{figure}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:}  $\mathbf{Y}=\{Y_n\forall n\}$, $L$, $s$, $C$, $\mathbf{B}^{(k)}=\{B^{(k)}(j)\forall j\}$, $k=1, 2$. 
				\STATE {\bf Output:} $I^{(k)}_n$, $k=1, 2$: set containing the indices of the chunks that can have their $n$th layer fetched over link $k$.
					
    \STATE  $deadline(i)=(i-1)L+s \quad \forall i$ 
     \STATE  $r^{(k)}(j)=\sum_{j^\prime=1}^{j} B^{(k)}(j^\prime)$, $j=1,....deadline(C)$, $k=1, 2$
    \FOR{each layer $n = 0, \cdots, N$}
     %{\bf j not defined - need efficient loop - should be also outside $n$ loop. }
    % available bandwidth on lte connection up to time $j, \forall j$
    \STATE $j_{1}=j_{2}=deadline(C)$
    \FOR{$i=C:-1:1$}
    \STATE $j_k =\min(j_k, deadline(i))$, $k=1, 2$
    	\IF{($n=0$ or $i \in I_{n-1}^{(1)}$ or $i \in I_{n-1}^{(2)})$}
    		\IF{$max(r^{(1)}(j_1), r^{(2)}(j_2)) \geq Y_n$}
      			\STATE $[R^{(k)},B2^{(k)}, j2^{(k)}, nf^{(k)}] = \bf{Backward}(i, j_k, \{r^{(k)}(j)\forall j\}, \mathbf{B}^{(k)}, Y_n)$, $k=1, 2$
      		%	\STATE $tmp^{(k)}=0$, $k=1, 2$% {\bf Anis, check $\infty$ or zero, since you will be doing max later. If not fetched and has infinite residual bandwidth, this will be chosen. }
      		%	\FOR{k=1:2}
      		%	\IF{$nf^{(k)}=0$}
      			\STATE $tmp(k)=(1-nf^{(k)})R^{(k)}(min(j2(k), deadline(i-1)))+r^{(3-k)}(deadline(i-1))$, $k=1, 2$
      		%	\ENDIF
      		%	\ENDFOR
      			\STATE $k_1=\arg\max \big(tmp^{(k)}\big)$
      			\IF { $(r^{(k_1)}(deadline(i)) \geq Y_n)$}
      				\STATE $I_n^{(k_1)}=I_n^{(k_1)} \cup i$
      				\STATE $\mathbf{B}^{(k_1)}=B2^{(k_1)}$, $j_{k_1}=j2^{(k_1)}$, $r^{(k_1)} =R^{(k_1)}$
      			\ENDIF
      		\ENDIF
	\ENDIF
      \ENDFOR
     \ENDFOR
   				\end{algorithmic}
				\caption{Offline MP-SVC Algorithm }\label{algo:mpsvc}
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}




\begin{figure}
		%\vspace{-.6in}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:} $i, j, r, B, Y_n$
					\STATE {\bf Output:} $R$ is the residual cumulative bandwidth at different times after fetching chunk $i$, $B2$ is the residual bandwidth after accounting for fetching of chunk $i$, $j2$ is the index at which chunk $i$ starts being fetched, $nf$ determines whether chunk $i$ can be fetched, 1 if it  can't be fetched. 
    \STATE {\bf Initialization:}
    \STATE $i=C$,  $nf=0$
    \IF{$r < Y_n$}
    	\STATE $nf=1$
	\ELSE
     \WHILE {($Y_n > 0$)}

            \STATE $fetched=min(B(j), Y_n)$ 
            \STATE $B(j)=B(j)-fetched$, $r(j)=r(j)-fetched$, $Y_n(i)=Y_n(i)-fetched$
	   \STATE {\bf if } {$(B(j)=0)$} {\bf then }  $j=j-1$            	
    \STATE $R=r$, $B2=B$, $j2=j$        
\ENDWHILE
\ENDIF
				\end{algorithmic}
				\caption { Backward Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}
\fi



{\bf Complexity Analysis}:  The algorithm sequentially decides  each layer one after the other, and thus it is enough to find the complexity of one layer to compute overall algorithm complexity. 
For each layer $n$, the algorithm first finds the cumulative bandwidth of every time slot $j$, $r^{(k)}(j)$ which is linear complexity. Then, it starts from the last chunk, and performs  the backward algorithm on each link at each time. The backward algorithm determines whether the chunk can be fetched in that link and the amount of residual bandwidth. Since the complexity of backward algorithm is linear in $C$, the overall complexity for a layer is $O(C^2)$. Thus, the overall complexity is $O(NC^2)$. 
 
 \begin{remark}
In our algorithm, with the use of $\gamma$, the lower layers have higher priority than the higher layers. 
%
%always prefer pushing {\em all} chunks to $n$th layer quality rather than fetching {\em some} chunks at $(n+1)$th and  {\em some}  others at $(n-1)$th qualities {\bf Vaneet: I re-wrote your statement, please check if it is better now}. 
The algorithm also prefers to utilize the excess bandwidth to fetch the later chunks rather than earlier chunks. Hence, our proposed algorithm reduces the un-necessary quality variation across neighboring chunks. 
\end{remark}

\begin{remark}\label{rem_mptcp}
We note that if one can use Multi-path TCP, the above algorithm can be used on only one path by assigning the sum of the bandwidths of the two links to this path and having the bandwidth of the other path as zero. The streaming algorithm that utilizes Multi-path TCP is denoted as MPTCP-SVC. Further, this algorithm  can be used for both AVC and SVC encoding since the decisions of the quality can be used with any of the encoding methods.  
\end{remark}

\begin{remark}
MPTCP-SVC will perform no worse than MP-SVC, since utilizing multipath TCP, each chunk will finish downloading no later than using MP-SVC. Thus, there will be a loss in performance as compared to the use of multipath TCP.
\end{remark}

\begin{remark} 
The algorithm can be easily  extended to the case when there are more than 2 links where  each layer of a chunk is assigned to the link that leaves more total residual bandwidth to the earlier chunks.
\end{remark}
 
 

==> skipperfect_E.tex <==
\subsection{Link Preference ($\gamma^{(m+1)} < \lambda < \gamma^{m}$)}
\label{skipalgoPref}

In this section, we describe our 
 proposed algorithm when one of the links need to be used less than the other one because one could be more expensive or less energy efficient. The algorithm is called ``Multi-Path-Pref SVC Algorithm" (MP-Pref-SVC).
 
 Initially, MP-Pref-SVC algorithm follows the same steps of MP-SVC up to the $m$th layer. Therefore, the fetching policy such that both links are equally likely to be used and maximum number of chunks that can be fetched up to $m$th layer quality level is found. However, up to this point, the decision did not consider minimizing the usage of link 1. To do so, forward algorithm (algorithm 4) is run in order to simulate fetching the layers according to the policy that was found using up to $m$th layer MP-SVC but with prioritizing fetching chunks on link 2. The algorithm starts from the base layer of the first chunk that was decided to be fetched, and checks the possibility of fetching it over link 2 first(lines $12-16$). If $k$th layer of chunk $i$ can't be totally fetched on link 2 before its deadline, it is assigned to link 1(lines $17-21$). Therefore, forward algorithm ensures that chunks can be fetched according to $m$th layer MP-SVC decision with minimum use of link 1.
 
 Since $\lambda > \gamma^{(m+1)} $, all layers starting from $(m+1)$th up to the highest layer can't be fetched on link 1; Otherwise, the objective is minimized instead of being maximized. Therefore MP-SVC still can be run for those layers but considering that the link 1 input bandwidth is only the amount that is needed to satisfy MP-SVC fetching policy up to the $m$th layer.  
 
 

\begin{figure}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE Run MP-SVC algorithm for layers $n=0$ to $m$
				\STATE $B^{(1)}$=forward($C, r^{(1)}, r^{(2)} B^{(1)}, B^{(2)}, Y_{1,...,m}(i), I_{1,...,m}^{(1)}, I_{1,...,m}^{(2)}$)
				\STATE Run MP-SVC algorithm for all layers. i.e $n=0$ to $N$
				   \end{algorithmic}
				\caption{Offline MP-Pref-SVC Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}


 
 \begin{figure}
		%\vspace{-.6in}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:} $C, r^{(1)}, r^{(2)} B^{(1)}, B^{(2)}, Y_n(i), I_n^{(1)}, I_n^{(2)},\quad n=1,...m$
					\STATE {\bf Output:} $R$ is the residual cumulative bandwidth at different times after fetching chunk $i$, $B2$ is the residual bandwidth after accounting for fetching of chunk $i$, $j2$ is the index at which chunk $i$ starts being fetched, $nf$ determines whether chunk $i$ can be fetched, 1 if it is can't be fetched. 
    \STATE {\bf Initialization:}
    \STATE $i=1$
    \STATE $j_k=1$
    \STATE $n=0$
    \STATE $B^{(k)}_{tmp}=B^{(k)}$, and $r^{(k)}_{tmp}=r^{(k)}$
    \WHILE{$(i \leq C)$}
    	\WHILE{$(n \leq m)$}
	 	\IF{$(i \in I_n^{(1)}$ or $i \in I_n^{(2)})$}
			\IF{($j$ is the first time in which layer $n$ of chunk $i$ is fetched)}
   				\IF{$(r^{(2)}_{tmp}(deadline(i))-r^{(2)}_{tmp}(j2) \geq Y_n(i)$}
   					\IF{$(i \in I_n^{(1)})$}
   						\STATE $I_n^{(2)}=I_n^{(2)} \cup i$
						\STATE $I_n^{(1)}=I_n^{(1)} \ \ i$
					\ENDIF
				\ELSIF{$(r^{(1)}_{tmp}(deadline(i))-r^{(1)}_{tmp}(j1) \geq Y_n(i)$}
					\IF{$(i \in I_n^{(2)})$}
						\STATE $I_n^{(1)}=I_n^{(1)} \cup i$
						\STATE $I_n^{(2)}=I_n^{(2)} \ \ i$
					\ENDIF
				\ENDIF
			\ENDIF
		\ENDIF
				
	   \IF{$(i \in I_n^{(k)})$}
            	\STATE $fetched=min(B^{(k)}_{tmp}(j_k), Y_n(i))$ 
            	\STATE $B^{(k)}_{tmp}(j_k)=B^{(k)}_{tmp}(j_k)-fetched$
		\STATE $r^{(k)}_{tmp}(j_k)=r^{(_k)}_{tmp}(j_k)-fetched$
	%\ELSIF{$(i \in I_n^{(1)})$}
            	%\STATE $fetched=min(B^{(1)}_{tmp}(j1), Y_n(i))$ 
            	%\STATE $B^{(1)}_{tmp}(j1)=B^{(1)}_{tmp}(j1)-fetched$, $r^{(1)}_{tmp}(j1)=r^{(1)}_{tmp}(j1)-fetched$
	\ENDIF
            
            \STATE $Y_n(i)=Y_n(i)-fetched$
	   \STATE {\bf if } {$(B(j_k)=0)$} {\bf then }  $j_k=j_k+1$, $k=1,2$
	     %\STATE {\bf if } {$(B(j1)=0)$} {\bf then }  $j1=j1+1$
	   %\STATE {\bf if } {$(Y_n(i)=0)$} {\bf then }  $n=n+1$
	   \IF{($(Y_n(i)=0)$)}
	   	   \STATE $n=n+1$
		   	\IF{$(n > m)$}
				\STATE $n=0$, $i=i+1$
			\ENDIF
	    \ENDIF
	   %\STATE {\bf if } {$(Y_n(i)=0)$} {\bf then }  $n=n+1$          	
   % \STATE $R=r$, $B2=B$, $j2=j$        
\ENDWHILE
\ENDWHILE
\STATE $B^{(1)}=B^{(1)}-B^{(1)}_{tmp}$
				\end{algorithmic}
				\caption { Forward Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}

Finally, we created MPTCP-Pref-SVC algorithm by aggregating both bandwidth up to the $m$th layer, and then applying modified version of forward algorithm where only the number of bytes that can't be fetched over link 2 are assigned to link 1. Therefore, in MPTCP forward algorithm a layer can be split into two links. i.e, part of it is fetched over one of the links and the remaining still can be fetched over the other link.
	
\subsubsection{Optimality of the MP-Pref-SVC}\label{optim_skip}

Since MP-Pref-SVC runs MP-SVC up to the $m$th layer, we know from section \ref{} that the optimality holds for the fetching policy of layers $1$ to $m$. Moreover, MP-SVC is run again for the layers $n=0$ to $N$, and if both link bandwidths that are passed to MP-SVC after $m$th layer are the optimal, the decisions of all layers must be optimal. Therefore, the only extra thing that needs to be investigated for the MP-Pref-SVC algorithm is the optimality of the $m$th layer forward algorithm. In other words, if $m$th layer forward algorithm finds the minimum link 1 bandwidth that needs to be used such that all decisions up to the $m$th layer are satisfied, then all the lemmas and the main theorem the proves the optimality of MP-SVC are applicable to MP-Pref-SVC, and the optimality of MP-Pref-SVC follows the same proof of the MP-SVC. The following lemma states the optimality of the $m$th layer forward algorithm.

\begin{lemma}%{Theorem}
Forward algorithm guarantees fetching all chunks according MP-SVC decisions up to the $m$th layer with minimum usage of link 1. In other words, the link 1 bandwidth that is found by calling forward algorithm is optimal, and no algorithm can achieve same fetching policy with less usage of link 1. 
\label{lem:mpPref}
\end{lemma}

